Modeling reputation-based behavioral biases in school choice

A fundamental component in the theoretical school choice literature is the problem a student faces in deciding which schools to apply to. Recent models have considered a set of schools of different selectiveness and a student who is unsure of their strength and can apply to at most $k$ schools. Such models assume that the student cares solely about maximizing the quality of the school that they attend, but experience suggests that students' decisions are also influenced by a set of behavioral biases based on reputational effects: a subjective reputational benefit when admitted to a selective school, whether or not they attend; and a subjective loss based on disappointment when rejected. Guided by these observations, and inspired by recent behavioral economics work on loss aversion relative to expectations, we propose a behavioral model by which a student chooses schools to balance these behavioral effects with the quality of the school they attend. Our main results show that a student's choices change in dramatic ways when these reputation-based behavioral biases are taken into account. In particular, where a rational applicant spreads their applications evenly, a biased student applies very sparsely to highly selective schools, such that above a certain threshold they apply to only an absolute constant number of schools even as their budget of applications grows to infinity. Consequently, a biased student underperforms a rational student even when the rational student is restricted to a sufficiently large upper bound on applications and the biased student can apply to arbitrarily many. Our analysis shows that the reputation-based model is rich enough to cover a range of different ways that biased students cope with fear of rejection, including not just targeting less selective schools, but also occasionally applying to schools that are too selective, compared to rational students.

==> paper_sections/intro-v01.tex <==
\section{Introduction}

Consider a student applying to college. Out of the thousands of schools in the US, which should she apply to? \todo{turn this into some kind of catchy hook}



Often the utility of students that apply to school consists of two components: 1. A standard consumption utility for a school they were admitted to and decided to attend; 2. a \emph{behavioral} utility that corresponds to a reputation gain from being admitted to a school or a reputation loss from being rejected from a school. 
The utility from the first component equals the maximal value of a school that the student was admitted to. The second utility is exhibited for each one of the schools that the student applies to. The rationale here is that this reptutational term is exhibited when the students get to see her application results or tell her friends about them and in a sense is independent from the results of her other applications.

This view fits well the spirit of a model of expectations-based reference-dependent preferences (EBRD) by K\H{o}szegi and Rabin~\cite{KR06, KR07, KR09}. In the EBRD model, the agent separately derives two forms of utility: the standard ``consumption utility'' and an additional reputational cost termed 'new utility' relative to a \emph{reference point} determined by her expectations about her environment. An agent with EBRD preferences will take into account how her strategy affects her expected outcome, and thus her reference point and gain-loss utility. \socomment{This was copied from Emily's background}

In the classic ERBD model the new cost is related to the consumption. Per the previous discussion, in our model we explicitly distinguish between the two. Let $v$ be the consumption value of some school, then we say that a student that is admitted to the school receives an $\rho \cdot v$ reputational utility for being admitted to the school regardless of whether she attends the school or not. As in the ERBD, reputation utility is relative to a reference point which is defined for each school as the expected reputational gain: $p\cdot \tau \cdot v$. If the student is admitted to the school it gains an extra reputational utility of $(1-p) \tau v$  while if it is rejected it incurs a reputational cost of $p \cdot \tau v$. Note that a rational agent that has these behavioral term behaves exactly the same as an agent that does not have them since the reputaional costs and benefit cancel out and will not affect her expected utility ($p\cdot(1-p) \tau v - (1-p)p\tau v = 0$). However, as anyone that was ever rejected knows rejections are much more potent than success, as in the celebrated line of work on prospect theory \cite{} on loss aversion. Propsect theory tells us that people tend to put more emphasis on their losses than their gains. The same assumption is also applied by the ERBD model. Hence, in this work we consider biased students that have loss aversion. We choose model loss aversion linearly and assume that a biased agent with loss parameter $\lambda>1$ has the following expected reputation utility $p\cdot(1-p) \tau v - \lambda(1-p)p\tau v = -\gamma(1-p)p v$. It will turn out to be convenient to set $\gamma = (1-\lambda)\cdot \tau$ and study the problem in terms of $\gamma$ instead.



\socomment{I think we need another parameter for this to make sense. So assume the reputations cost is $\rho$ times the consumption value. We can get rid of this parameter at the same time we use $\gamma$ instead of $\alpha$ and $\beta$. Also instead of having $\alpha$ and $\beta$ I switched it to $1$ and $\lambda$ which seems somewhat simpler. }

